NEWTON: Are Large Language Models Capable of Physical Reasoning?

Large Language Models (LLMs), through their contextualized representations, have been empirically proven to encapsulate syntactic, semantic, word sense, and common-sense knowledge. However, there has been limited exploration of their physical reasoning abilities, specifically concerning the crucial attributes for comprehending everyday objects. To address this gap, we introduce NEWTON, a repository and benchmark for evaluating the physics reasoning skills of LLMs. Further, to enable domain-specific adaptation of this benchmark, we present a pipeline to enable researchers to generate a variant of this benchmark that has been customized to the objects and attributes relevant for their application. The NEWTON repository comprises a collection of 2800 object-attribute pairs, providing the foundation for generating infinite-scale assessment templates. The NEWTON benchmark consists of 160K QA questions, curated using the NEWTON repository to investigate the physical reasoning capabilities of several mainstream language models across foundational, explicit, and implicit reasoning tasks. Through extensive empirical analysis, our results highlight the capabilities of LLMs for physical reasoning. We find that LLMs like GPT-4 demonstrate strong reasoning capabilities in scenario-based tasks but exhibit less consistency in object-attribute reasoning compared to humans (50% vs. 84%). Furthermore, the NEWTON platform demonstrates its potential for evaluating and enhancing language models, paving the way for their integration into physically grounded settings, such as robotic manipulation. Project site: https://newtonreasoning.github.io

==> sections/old_stuff.tex <==
This track aims to measure the distribution differences between human's and language models' comprehension of object attributes. Questions within this category are identical to those exposed to human annotators, with minimal modifications to suit the prompting format of different models.  The \textit{Explicit Deduction} track aims to assess language model's ability to apply their understanding of object attributes in explicit reasoning tasks. This involves reasoning about whether certain statements about object attributes are correct, which object is distinctly different from others based on a particular attribute, etc. The \textit{Implicit Induction} track aims to assess language model's ability to reason in scenario tasks, where the attribute to reason about is not mentioned explicitly.


However, development of an evaluation scheme for physical reasoning is challenging due to the absence of paired object-attribute data. Humans possess rich knowledge of the internal structure of objects and how they interact with the real world. Yet, such knowledge is typically captured in an implicit manner, and there lacks an explicit avenue for representing such information. Existing investigations in the physical reasoning domain, such as \cite{bisk2020piqa, arocaouellette2021prost} focus on common-sense reasoning, or small-scale validation, and hence diverse and systematic assessment for physical reasoning remains an open problem.

% benchmark proves useful for evaluating language models' understanding of underlying physics principles that dictate the behavior and properties of objects in everyday scenarios

% First, the \dataset \textcolor{Fuchsia}{\textbf{benchmark}} introduces a new suite of tasks aimed at physics reasoning that is easy for humans, but difficult for state-of-the-art instructed language models. Second, 



% comprises of three components: a dataset of objects and their physical attributes, a pipeline for systematic generation of questions for evaluating language models' physical reasoning under any user-designed scenario, a dataset of pre-generated questions for zero-shot prompting. Through progressively challenging tasks spanning foundational attribute understanding, explicit reasoning, and implicit scenario-based reasoning, the benchmark proves useful for evaluating language models' understanding of underlying physics principles that dictate the behavior and properties of objects in everyday scenarios.

% By employing physical reasoning, we can make informed predictions, solve problems, and devise strategies for designing and manipulating various physical systems.

% world sense
%  Definition of physical reasoning

% However, existing investigations in the physical reasoning domain, such as \cite{bisk2020piqa, arocaouellette2021prost} predominantly focus on common-sense reasoning or have limited question scope and diversity. Consequently, assessing the performance of language models in diverse and systematic physical reasoning tasks remains challenging.

% Development of an evaluation scheme for physical reasoning is challenging due to the absence of paired object-attribute data. Humans possess rich knowledge of the internal structure of objects and how they interact with the real world. However, there lacks an explicit avenue for representing such information. Works have explored leveraging 



% -- which is typically illustrated in an implicit manner. 




% with a large-scale repository of multi-human validated physical attribute annotations of everyday objects. \dataset is designed to assist with evaluation of the physical reasoning ability of language models, particularly regarding the attributes that govern everyday objects. 



% However, while the performance of language models in these domains have been extensively explored, the physical reasoning ability of such models, particularly regarding the understanding of fundamental physics attributes that govern everyday objects, remain largely under explored. 

% To address this gap, we propose the \dataset benchmark, designed to evaluate the physical reasoning capability of language models in a zero-shot manner. \dataset comprises of three components: a dataset of objects and their physical attributes, a pipeline for systematic generation of questions for evaluating language models' physical reasoning under any user-designed scenario, a dataset of pre-generated questions for zero-shot prompting. Through progressively challenging tasks spanning foundational attribute understanding, explicit reasoning, and implicit scenario-based reasoning, the benchmark proves useful for evaluating language models' understanding of underlying physics principles that dictate the behavior and properties of objects in everyday scenarios.






% Recent advancements in the field of 
% Workflow:
% - Rapid advancements in NLP, wide adoptions in tangent fields, more recently robotics.
% - Taking an object-centric view, we want to understand whether language models possess an ability to understand objects and their physical attributes.
% - However, 


% With the rapid advancements in the 

% Main contributions:
% \begin{itemize}
%     \item A new benchmark for zero-shot assessment of the ability for Large-Language Models to reason about the physics properties of everyday objects.
%     \item An assessment of existing LLM models using the benchmark
%     \item An evaluation on the effective prompting methods for evaluating in the context of physics reasoning.
% \end{itemize}

% In this paper, we introduce \dataset, a \textcolor{Aquamarine}{\textbf{repository}} of labeled object-centric data, a \textcolor{BurntOrange}{\textbf{pipeline}} for generating infinite evaluation scenarios, and a \textcolor{Fuchsia}{\textbf{benchmark}} with 160k QA-template questions. The \textcolor{Aquamarine}{\textbf{repository}} of object-attribute pairs is crowdsourced and filtered based 

% Intro
% Problem: 
% 1. Limited analysis of language models and their ability to reason in a physical context.
% 2. Limited data which is in an object-centric manner.
% 3. 
% Limited analysis of language models from an object centric view due to inavailablility of large-scale datasets / data which includes human intuition. 

% Why do we need newton: 
% 1. Object-attribute pairs to enable generation of personalized evaluation schemes in the context of physical reasoning
% 2. Recommendations and guidelines for generating templates.
% 3. Large-scale QA dataset to enable systematic evaluation of language models from three areas: fundational attribute understanding, explicit reasoning, and implicit reasoning.
% 4. Suggestions for improving language models in solving scenario-based tasks (finetuning, function calls)


% pipeline for generating personalized evaluation schemes, systematic evaluation of language models, improvement of language models (finetuning, function call, etc.),

% The annotation process involved utilizing a likert-scale setup to gather accurate ground truth annotations for object-attribute pairs. Annotators were presented with a 3-point scale and tasked with selecting the most suitable option to represent the given pair. The use of a likert scale allowed for simplicity and represented the extremes of the attribute conditions. The annotation interface aimed to collect responses that facilitated the categorization of data into opposing groups. To ensure reliability and consistency, a minimum of four annotators contributed overlapping annotations for each object-attribute pair. Each annotation task included a question specifying the object category and attribute, a set of 10 randomly-sampled images illustrating common objects within the category, and three answer choices. The annotators were prompted to focus on the textual category, with the inclusion of thumbnail visualizations for reference. This process resulted in the collection of 20,000+ annotations, which were later filtered to obtain over 2,700 unique and consistent object-attribute pairs.

% The dataset is curated based on the workflow illustrated in Figure \ref{fig:template_generation_pipeline}. The process starts with crowdsourcing human annotations on object attributes, which is then filtered based on inter-annotator agreement. Inter-annotator agreement is calculated as a percentage of annotators who agreed on the majority response of each object-attribute task. Each task consists of a minimum of four overlapping annotations, which is aggregated and used to compute the inter-annotator agreement score. The data is filtered to enforce a minimum of 0.75 annotator agreement, the data of which makes up the \dataset Repository.

% The filtered data is used to automatically populate the set of pre-defined templates, based on the attribute conditions associated with the templates. 


% \noindent \textbf{Annotation Filtering.} 

% Each question template has associated object slots and attribute conditions, as shown in Figure X. The attribute conditions are defined as $\{attribute, polarity\}$, where $attribute$ defines the physics attribute to group using, $polarity$ defines whether the highest or lowest extremity to use. The goal is to fill the pre-allocated slots with $n$ objects, chosen in accordance with the provided attribute condition.

% \section{Experimental Design}


% \subsection{Unifying the Format.} Different models require different variations of prompt input, and the unsuitable prompt could lead to an inaccurate assessment of the capability of language models. Hence, we adapt the question template for different families of models to adhere to the most effective prompting strategy.



% \begin{table}[htbp]
% \centering
% \begin{tabular}{c|c|c|c|}
% \hline
% \multirow{8}{*}{Foundational Attribute Understanding} & Task & Category & Template \\
% \cline{2-3}
% & Task 1 & Category 1 & Template 1 \\
% \cline{2-3}
% & Task 2 & Category 2 & Template 2 \\
% \cline{2-3}
% & Task 3 & Category 3 & Template 3 \\
% \cline{2-3}
% & Task 4 & Category 4 & Template 4 \\
% \cline{2-3}
% & Task 5 & Category 5 & Template 5 \\
% \cline{2-3}
% & Task 6 & Category 6 & Template 6 \\
% \cline{2-3}
% & Task 7 & Category 7 & Template 7 \\
% \hline
% \multirow{6}{*}{Explicit Reasoning} & Task & Category & Template \\
% \cline{2-3}
% & Task 1 & Category 1 & Template 1 \\
% \cline{2-3}
% & Task 2 & Category 2 & Template 2 \\
% \cline{2-3}
% & Task 3 & Category 3 & Template 3 \\
% \cline{2-3}
% & Task 4 & Category 4 & Template 4 \\
% \cline{2-3}
% & Task 5 & Category 5 & Template 5 \\
% \hline
% \multirow{9}{*}{Implicit Scenarios} & Task & Category & Template \\
% \cline{2-3}
% & Task 1 & Category 1 & Template 1 \\
% \cline{2-3}
% & Task 2 & Category 2 & Template 2 \\
% \cline{2-3}
% & Task 3 & Category 3 & Template 3 \\
% \cline{2-3}
% & Task 4 & Category 4 & Template 4 \\
% \cline{2-3}
% & Task 5 & Category 5 & Template 5 \\
% \cline{2-3}
% & Task 6 & Category 6 & Template 6 \\
% \cline{2-3}
% & Task 7 & Category 7 & Template 7 \\
% \cline{2-3}
% & Task 8 & Category 8 & Template 8 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table*}[t]
%   \centering
%   \caption{Question Types and Categories}
%   \begin{tabular}{p{4cm}ll}
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{Question Type}} & \multirow{2}{*}{Category Template} & \multicolumn{1}{c}{Section} \\
%     \multicolumn{1}{c}{} & & \multicolumn{1}{c}{(Question Type)} \\
%     \midrule
%     \multirow{3}{*}{Foundational Attribute Comprehension} & \multirow{3}{*}{Category 1} & Explicit Deduction \\
%     & & Implicit Induction \\
%     & & Other Subcategories \\
%     \midrule
%     \multirow{3}{*}{Explicit Deduction} & \multirow{3}{*}{Category 2} & Foundational Attribute Comprehension \\
%     & & Implicit Induction \\
%     & & Other Subcategories \\
%     \midrule
%     \multirow{3}{*}{Implicit Induction} & \multirow{3}{*}{Category 3} & Foundational Attribute Comprehension \\
%     & & Explicit Deduction \\
%     & & Other Subcategories \\
%     \bottomrule
%   \end{tabular}
% \end{table*}





% \begin{table}[ht]
% \centering
% \caption{Model Parameters and Data}
% \label{tab:model_parameters_data}
% \begin{tabularx}{\columnwidth}{Xcc}
% \toprule
% \textbf{Model} & \textbf{Parameters} & \textbf{Data} \\
% \midrule
% Flan-Alpaca-GPT4-XL & 3B & Flan, GPT4-Alpaca \\
% Model B & 200 & Dataset Y \\
% Model C & 150 & Dataset Z \\
% \bottomrule
% \end{tabularx}
% \end{table}

% \begin{table}[ht]
% \centering
% \caption{Model Parameters and Data}
% \label{tab:model_parameters_data}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Model} & \textbf{Parameters} & \textbf{Data} \\
% \midrule
% Flan-Alpaca-GPT4-XL & 3B & Flan, GPT4-Alpaca \\
% Model B & 200 & Dataset Y \\
% Model C & 150 & Dataset Z \\
% \bottomrule
% \end{tabular}
% \end{table}

% \noindent \textbf{GPT \cite{brown2020language}} is a model which processes text in a left-to-right fashion, pre-trained using  

% \noindent \textbf{Flan-T5} is based on the T5 (Text-to-Text Transfer Transformer) model and instruction-tuned using the Flan method.


% A popular encoder-decoder model known as T5 (Text-to-Text Transfer Transformer) is one such model that was subsequently fine-tuned via the Flan method to produce the Flan-T5 family of models. Flan-T5 is an instruction-tuned model and therefore is capable of performing various zero-shot NLP tasks, as well as few-shot in-context learning tasks. With appropriate prompting, it can perform zero-shot NLP tasks such as text summarization, common sense reasoning, natural language inference, question answering, sentence and sentiment classification, translation, and pronoun resolution. The examples provided in this post are generated with the Flan-T5 family.

% \noindent \textbf{Alpaca} \cite{alpaca} is a language model fine-tuned from LLaMA \cite{touvron2023llama} using 52K instruction following data generated using methods from Self-Instruct \cite{wang2023selfinstruct}. 

% \noindent \textbf{Dolly 2.0} is a language model based on the EleutherAI Pythia Model, and finetuned on a 15 000 human-generated prompt-response pairs.

% \noindent \textbf{Flan-T5}

% \noindent \textbf{GPT-4}

% \noindent \textbf{XLM-RoBERTa}

% \noindent \textbf{BERT}

% \textbf{RoBERTa}




% \dataset 

% aids with three facets : 

% \dataset comprises of three main components:
% (1) A large-scale dataset of human-annotated and validated object-attribute pairs.
% (2) A pipeline for systematic generation of personalized evaluation scenarios.
% (3) A large-scale dataset of QA questions to assess the ability of language models from three tracks: fundamental attribute understanding, explicit reasoning, and implicit reasoning of object attributes.

% \subsection{Object-Attribute Dataset}

% \subsection{QA Dataset}

% Data is collected through a combination of human annotation and automated template formatting, which will be outlined in Section X.

As well, the multiple-choice style question  attributes identifies objects that diverge distinctly from others based on a particular attribute, and more.

% Through grounding attributes to scenarios, his track presents a unique challenge, requiring models to engage in implicit induction to derive the attribute-based reasoning. We show examples of templates 



% through a combination of direct approximation and GPT-4 assisted grouping. Objects are then filtered for applicability to 

% explicit annotations of object-attribute pairs at a scale unmatched by other works. Further, the scale of questions provided in the 
% Discuss

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{sections/images/data_statistics_full.png}
%     \caption{Caption}
%     \label{fig:dataset-statistics}
% \end{figure*}

% \begin{itemize}
%     \item Distribution of questions within each task when looking at the attribute dimension
%     \item Downsampling to create a more balanced dataset
%     \item Potential to extend the dataset to alternative scenarios, since attributes are provided
% \end{itemize}





% \begin{table}[htbp]
%   \centering
%   \caption{Dataset Comparison}
%   \label{tab:dataset_comparison}
%   \begin{tabular}{|l|c|c|}
%     \hline
%     \rowcolor[HTML]{EFEFEF}
%     \textbf{Factors} & \textbf{Dataset 1} & \textbf{Dataset 2} \\
%     \hline
%     Factor 1 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 2 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 3 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 4 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 5 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 6 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%     Factor 7 & \cellcolor{red!50}\textcolor{white}{\textbf{X}} & \cellcolor{green!50}\textcolor{white}{\textbf{\checkmark}} \\
%     \hline
%   \end{tabular}
% \end{table}

% \begin{table}[h]
% \centering
% \begin{tabularx}{\textwidth}{|l|l|X|X|}
% \hline
% \textbf{Property} & \textbf{Type} & \textbf{Definition} & \textbf{Question} \\
% \hline
% Elasticity & Physics & Elasticity in this context refers to the ability of an object to recover to the original form after deformation. & If you were to deform \textless MASK\textgreater\ (by squeezing, hitting, etc.), can it recover to its original form? \\
% \hline
% Surface smoothness & Physics & Surface smoothness in this context refers to the texture of the outer surface of the object. & What is the surface smoothness of \textless MASK\textgreater? \\
% \hline
% Surface Hardness & Physics & Surface hardness in this context refers to the ability of a surface to resist damage. & How resistant to scratches or bruises is the surface of \textless MASK\textgreater? \\
% \hline
% Brittleness & Physics & Brittleness in this context refers to the resistance of objects to sudden forces. & How easy is it for \textless MASK\textgreater\ to break (shatter, crack) when a sudden impact force is applied? \\
% \hline
% Softness & Physics & Softness refers to the fluffiness and squishiness of the external and internal composition of an object. & What is the softness (fluffiness, squishiness) of \textless MASK\textgreater? \\
% \hline
% Sharpness & Physics & Sharpness refers to the exterior design and material of an object. & What is the sharpness of \textless MASK\textgreater? \\
% \hline
% Stiffness & Physics & Stiffness refers to whether an object can withstand continued force without deforming or cracking. & What is the amount of continued weight that \textless MASK\textgreater\ can withstand before deforming or cracking? \\
% \hline
% Malleability & Physics & Malleability refers to whether an object can be reshaped to take other geometries. & Can \textless MASK\textgreater\ be reshaped into other forms? \\
% \hline
% \end{tabularx}
% \caption{Properties of Objects}
% \label{tab:object_properties}
% \end{table}





% and based on inter-annotator agreement

% Have an agreement plot, depicting how many annotations agree under what percentage (maybe pie plot).

% \subsection{Dataset Statistics}


% \subsection{Benchmark Tracks} 







% Things to discuss here:
% * Benchmark tracks: Foundational Attribute Comprehension, Explicit Deduction, Implicit Induction
% * Statistics of dataset: how many objects, how many attributes, how many task types, question types (mc, boolean), how many questions in total.
% * Data collection process?


% \dataset is a benchmark designed to prompt language models to evaluate their ability to reason about physics attributes in a zero-shot manner. The dataset consists of X non-repeating questions, covering 8 attributes and 700 different object categories. 

% \subsection{Tasks}


% aimed at evaluating the physics reasoning capability of large language models. The benchmark addresses three tasks: human-like understanding, explicit reasoning, and implicit reasoning.

% We categorize the physics reasoning ability into two tiers: explicit reasoning, and implicit reasoning. Explicit reasoning refers to exposing the language model to the physics attribute that 
% \subsection{Tasks for Evaluating Physics Reasoning}



% We introduce \dataset, a large-scale dataset for prompting language models in a zero shot manner. \dataset provides X questions across Y object categories and 8 physics attributes. In this section, we provide an overview of the dataset collection method and assessment of the dataset statistics. 

% \subsection{Dataset Collection}
% Dataset collection involves three main stages, namely attribute annotation, annotation filtering, and question template formatting.

% \noindent \textbf{Attribute Annotation.} 
% - crowdsourced
% - 8 physics attributes
% - 742 categories


% \noindent \textbf{Annotation Filtering.} 
% - filter annotations based on annotator agreement
% - only keep highly confident annotations
% - only keep the annotations which are at the extreme ends of the spectrum

% \noindent \textbf{Question Template Formatting.} 
% - different types of templates
% - different phrasing for different models (masked vs. generative)

% It is hypothesized that with the rich set of object-attribute pairs which \dataset provides, we can endow language models with physical reasoning by finetuning in an explicit manner, such that performance for downstream implicit tasks is improved. To test this hypothesis, we fine-tune the base BERT model for the multiple choice task. The baseline consists of the base BERT model \cite{devlin2019bert}, fine-tuned on the SWAG dataset for multiple choice inference \cite{zellers2018swag}. The finetuning process uses subsets of \dataset QA - explicit reasoning track \{5000, 10000, 40000\}, and all models are evaluated on the implicit reasoning task, provided by the \dataset QA Implicit Reasoning Track. As shown in Figure \ref{fig:ablation} e find that including \dataset as a part of the pre-training procedure vastly improves performance on downstream implicit reasoning tasks, demonstrating the potential of leveraging \dataset for finetuning language models to improve their physical reasoning ability.

% \noindent \textbf{Polarity and Position Bias in Language Models.} To investigate whether different polarities of questions impact model performance, we use \dataset Benchmark - Track 2, and separate prompting questions into Positive and Negative polarity. Positive polarity questions refer to {is, is more, is the most}, while negative polarity questions refer to {is not, is less, is the least} style questions, from Table \ref{tab:question_samples}. In comparing model accuracy differences, we find that most models have consistent performance for both polarities, with X exhibiting the smallest difference of X, and Flan-T5-Base exhibiting the largest difference of X. To investigate bias by position, we grouped questions by the position of the ground truth answer, the plot of which is shown in Figure \ref{fig:accuracy-position}. The model which exhibits the least variance in accuracy grouped by position is X, while the model with the most variance is X.




% Also, we note the gap between inter-human agreement percentage between human responses and language model responses for the identical set of questions. We also find a high 

% While some models excelled at understanding particular attributes, most statistics approximated that of a random baseline. Out of all examined models, GPT-4 achieved the highest overall accuracy and surpassed other language models across the majority of attributes, showing potential for emergent understanding of physics attributes.


% \noindent \textbf{Instruction-Tuned Models understand physics attributes better than Masked models.} It is anticipated that fine-tuning on query-answer pairs will enhance the physics attribute understanding and reasoning ability of language models. 

% \noindent \textbf{Language Models are better at boolean reasoning than multiple choice (4 choices) reasoning.} 

% \noindent \textbf{There is a gap between human and language model knowledge across the majority of physics attributes.} 

% \noindent \textbf{Fundamental Understanding.} In analyzing the performance of several language models 

% \begin{table*}[t]
%     \centering
%     \caption{\textbf{Model Comparison: Language Model Performance}}
%     \resizebox{1.0\textwidth}{!}{%
%     \begin{tabular}{c|cccccccc}
%         \toprule
%         \rowcolor[HTML]{CBCEFB}
%         \multirow{2}{*}{\textbf{Language Models}} & \multicolumn{8}{c}{\textbf{Features}} \\
%         \cmidrule{2-9}
%          & \textbf{Elasticity} & \textbf{Surface Smoothness} & \textbf{Surface Hardness} & \textbf{Brittleness} & \textbf{Softness} & \textbf{Sharpness} & \textbf{Stiffness} & \textbf{Malleability} & \textbf{Overall Accuracy} \\
%         \midrule
%         \rowcolor[HTML]{FBE0CB}
%         \multicolumn{9}{l}{\textbf{GPT-3.5}} \\
%         \midrule
%         GPT-3.5 & & & & & & & & \\
%         \rowcolor[HTML]{EFEFEF}
%         \multicolumn{9}{l}{\textbf{GPT-4}} \\
%         \midrule
%         GPT-4 & & & & & & & & \\
%         \rowcolor[HTML]{FBE0CB}
%         \multicolumn{9}{l}{\textbf{BERT}} \\
%         \midrule
%         BERT & & & & & & & & \\
%         \rowcolor[HTML]{EFEFEF}
%         \multicolumn{9}{l}{\textbf{RoBERTa}} \\
%         \midrule
%         RoBERTa & & & & & & & & \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[t]
% \begin{center}
%     \resizebox{\textwidth}{!}{%z
%     \begin{tabular}{l p{0.6pt}ccccccccc}
%     \toprule
%      Task& & \multicolumn{9}{c}{Press (\emph{Acc.\%})}\\
%     \cline{3-13}
%     Personalized object&& Computer mouse & Minecraft torch & Buzzer && LEGO train & 8 ball  & Drawer && Queen piece & Plastic bowl & Takeaway bag \\
%     \midrule
%     Simulation &&  13.3 & 6.7&30.0 &&13.3 &20.0 &3.3&&3.3&20.0 &16.7 \\
%     VR interface (w/o personalized objects)&& 3.3 & 6.7& 16.7&& 13.3 & 10.0 & 3.3&& 0.0& 16.7&13.3 \\
%     VR interface (with personalized objects)&& 60.0 & 63.3 & 83.3 && 30.0 & 70.0 & 40.0 && 46.7 & 56.7 & 60.0\\
%        AR2-D2 (Ours) &&56.7 & 53.3 & 73.3 && 50.0 &55.7 &23.3 && 46.7 &53.3 & 63.3\\
%     \bottomrule
    
%     \end{tabular}
%     }
% \end{center}
% \caption{\textbf{Task test results}.We utilized AR2-D2 to collect demonstrations and train BC agents for real robot deployment. Our observations revealed comparable results between our data collection approach and alternative methods. Success rates (mean \%) of the foundational skills tested on personalized objects collected via AR2-D2. For each skill, we evaluated it across ten different sets of distractors with the target object and repeated thrice for consistency. The result has shown that our data collection approach with minimal fine-tuning achieves comparable results to real-world data collected on these personalized objects via PerAct's VR interface with a physical robot.}
% \label{tab:press_push_pick_table}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
%     \toprule
%      \textbf{Language Model} & & \multicolumn{3}{c}{\textbf{Elasticity}} && \multicolumn{3}{c}{\textbf{Surface Smoothness}} && \multicolumn{3}{c}{\textbf{Surface Hardness}} \\
%     \cline{3-5}\cline{7-9}\cline{11-13}
%     && Attribute 1 & Attribute 2 & Attribute 3 && Attribute 4 & Attribute 5 & Attribute 6 && Attribute 7 & Attribute 8 & Attribute 9 \\
%     \midrule
%     \textbf{GPT-3.5} &&  0.82 & 0.75 & 0.88 && 0.91 & 0.84 & 0.77 && 0.79 & 0.83 & 0.88 \\
%     \textbf{GPT-4} && 0.85 & 0.87 & 0.91 && 0.83 & 0.89 & 0.87 && 0.88 & 0.92 & 0.85 \\
%     \textbf{BERT} && 0.77 & 0.81 & 0.79 && 0.86 & 0.83 & 0.75 && 0.78 & 0.80 & 0.83 \\
%     \textbf{RoBERTa} && 0.88 & 0.92 & 0.85 && 0.81 & 0.87 & 0.89 && 0.90 & 0.88 & 0.93 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{center}
% \caption{\textbf{Object Attributes of Language Models}. This table presents the evaluations of different language models on various object attributes. The attributes include elasticity, surface smoothness, and surface hardness. Each attribute is represented by three sub-attributes (Attribute 1, Attribute 2, and Attribute 3 for elasticity, Attribute 4, Attribute 5, and Attribute 6 for surface smoothness, and Attribute 7, Attribute 8, and Attribute 9 for surface hardness). The language models are compared based on their performance scores for each attribute and sub-attribute.}
% \label{tab:language_model_attributes}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
%     \toprule
%      \textbf{Language Model} && \multicolumn{9}{c}{\textbf{Agreement \%}} \\
%     \cline{3-13}
%     && Elasticity & Stiffness & Surface Smoothness && Surface Hardness & Softness & Brittleness && Malleability & Sharpness & Overall \\
%     \midrule
    
%     \textbf{dolly-v2-7b} && 23.7  &  11.7  &  4.1  &&  3.5  &  1.3  &  1.3  &&  8.6  &  2.5  &  7.6  \\
% \textbf{flan-alpaca-gpt4-xl} && 9.3  &  1.1  &  59.7  &&  19.9  &  25.1  &  6.1  &&  9.5  &  7.4  &  15.2  \\
% \textbf{flan-t5-small} && 0.0  &  0.0  &  0.0  &&  0.0  &  0.0  &  0.0  &&  0.0  &  0.0  &  0.0  \\
% \textbf{flan-t5-base} && 79.8  &  45.9  &  61.9  &&  28.1  &  25.4  &  6.1  &&  77.0  &  4.7  &  41.7  \\
% \textbf{flan-t5-large} && 0.0  &  0.4  &  61.9  &&  30.1  &  25.4  &  6.1  &&  9.8  &  4.1  &  13.7  \\
% \textbf{flan-t5-xl} && 9.3  &  4.4  &  15.6  &&  42.4  &  59.9  &  6.1  &&  9.9  &  54.6  &  27.5  \\

% \textbf{unifiedqa-v2-t5-large-1363200} && 0.0  &  0.0  &  61.9  &&  30.5  &  10.2  &  6.1  &&  9.5  &  23.5  &  14.3  \\
% \textbf{alpaca-lora-7b} && 9.3  &  0.0  &  44.3  &&  0.6  &  14.4  &  3.9  &&  9.5  &  1.9  &  10.0  \\
% \textbf{gpt\_turbo} && 22.5  &  0.0  &  0.7  &&  13.5  &  6.6  &  6.2  &&  58.8  &  1.1  &  16.4  \\
% \textbf{gpt4} && 51.3  &  8.0  &  14.1  &&  47.1  &  59.5  &  76.5  &&  44.1  &  58.4  &  49.7  \\
% \midrule 
% \textbf{Average} && 20.5 & 7.2 & 32.4 && 21.6 & 22.8 & 11.8 && 23.7 & 15.8 & 19.6 \\


%     \midrule
%     \textbf{Human} && 89.1 & 78.7 & 79.2 && 78.9 & 89.4 & 82.6 && 86.8 & 90.5 & 84.4 \\

%     % \textbf{Model W} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     % \textbf{Model V} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{center}
% \caption{\textbf{Foundational attribute understanding.}.}
% \label{tab:fundamental_attribute_understanding}
% \end{table*}


% \begin{table*}[t]
% \begin{center}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
%     \toprule
%      \textbf{Language Model} && \multicolumn{9}{c}{\textbf{Agreement \%}} \\
%     \cline{3-13}
%     && Elasticity & Stiffness & Surface Smoothness && Surface Hardness & Softness & Brittleness && Malleability & Sharpness & Overall \\
%     \midrule
    
%     % \textbf{xlnet-large-cased} && 38.3 & 32.7 & 31.5 && 31.1 & 39.1 & 28.6 && 35.5 & 27.6 & 33.8 \\
%     % \textbf{xlm-roberta-large} && 37.1 & 23.1 & 33.6 && 21.5 & 36.7 & 40.6 && 32.2 & 23.1 & 32.3 \\
%     % \textbf{roberta-large} && 27.0 & 24.4 & 37.7 && 22.6 & 37.4 & 48.6 && 34.5 & 34.8 & 34.5 \\
%     % \textbf{bert-large-uncased} && 32.9 & \textbf{42.2} & 28.1 && 39.8 & 38.6 & 25.0 && 23.9 & 31.1 & 31.7 \\
%     % \textbf{albert-xxlarge-v2} && 36.4 & 27.9 & \textbf{41.1} && 26.9 & 41.3 & 8.3 && 18.6 & 23.4 & 27.9 \\
%     % \textbf{Flan-T5-small} && - & - & - && - & - & - && - & - & - \\
%     \textbf{Flan-T5-Base} && 88.8 & 58.6 & \textbf{78.6} && 36.7 & 28.8 & 7.5 && \textbf{87.8} & 5.2 & 48.5 \\
%     \textbf{Flan-T5-Large} && 0.0 & 0.5 & \textbf{78.6} && 39.1 & 28.8 & 7.5 && 12.2 & 4.6 & 16.6 \\
%     \textbf{Flan-T5-XL} && 11.2 & 5.4 & 19.1 && 53.9 & 66.3 & 7.5 && 12.4 & 59.6 & 31.3 \\
%     \textbf{Flan-alpaca-GPT4-XL} && 11.2 & 3.4 & 76.8 && 27.3 & 29.8 & 7.5 && 12.0 & 8.2 & 18.9 \\
%     \textbf{Dolly-v2-7b} && - & - & - && - & - & - && - & - & - \\
%     \textbf{UnifiedQA-T5-large} && 0.0 & 0.0 & \textbf{78.6} && 39.1 & 11.4 & 7.5 && 12.0 & 26.0 & 17.2 \\
%     \textbf{alpaca-lora-7b} && 11.2 & 0.0 & 56.4 && 0.8 & 16.4 & 4.6 && 12.0 & 2.8 & 12.2 \\
%     % \textbf{falcon-7b-instruct} && - & - & - && - & - & - && - & - & - \\
%     \textbf{GPT-3.5-turbo} &&  26.0 & 0.0 & 0.9 && 16.4 & 7.5 & 7.0 && 67.6 & 1.2 & 18.9 \\
%     \textbf{GPT-4} && \textbf{57.8} & \textbf{63.5} & 18.2 && \textbf{60.9} & \textbf{66.5} & \textbf{92.5} && 50.6 & \textbf{64.8} & \textbf{61.1} \\
%     \midrule
%     \textbf{Human} && \textbf{89.1} & \textbf{78.7} & 79.2 && \textbf{78.9} & \textbf{89.4} & \textbf{82.6} && 86.8 & \textbf{90.5} & \textbf{84.4} \\

%     % \textbf{Model W} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     % \textbf{Model V} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{center}
% \caption{\textbf{Foundational attribute understanding.}.}
% \label{tab:fundamental_attribute_understanding}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
% \toprule
% \textbf{Language Model} && Elasticity & Stiffness & Surface Smoothness && Surface Hardness & Softness & Brittleness && Malleability & Sharpness & Overall \\
% \cline{3-13}
%   && \multicolumn{9}{c}{\textbf{Boolean (overall/positive/negative)}} \\

% \midrule



% \textbf{dolly-v2-7b} && 30.2 & 25.1 & 27.2 && 31.5 & 28.9 & 24.6 && 26.1 & 26.7 & 27.5 \\
% \textbf{flan-alpaca-gpt4-xl} && 54.9 & 61.5 & 49.8 && 59.5 & 58.1 & 49.2 && 48.8 & 68.1 & 56.3 \\
% \textbf{flan-t5-large} && 42.7 & 40.5 & 44.3 && 21.0 & 50.6 & 30.3 && 38.9 & 52.2 & 40.4 \\
% \textbf{flan-t5-xl} && 61.4 & 60.4 & 50.5 && 65.3 & 74.0 & 51.4 && 59.2 & 78.8 & 62.9 \\
% \textbf{flan-t5-base} && 56.0 & 52.2 & 48.2 && 49.1 & 52.1 & 49.6 && 50.2 & 54.6 & 51.6 \\
% \textbf{unifiedqa-v2-t5-large} && 46.6 & 51.7 & 49.8 && 57.4 & 61.1 & 50.6 && 49.7 & 54.5 & 52.7 \\
% \textbf{flan-t5-small} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{alpaca-lora-7b} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{falcon-7b-instruct} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-3.5-turbo} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-4} && - & - & - && - & - & - && - & - & - \\

% \midrule
%  && \multicolumn{9}{c}{\textbf{Multiple Choice (overall/positive/negative)}} \\
%  \midrule

%  \textbf{dolly-v2-7b} && 42.4 & 44.2 & 42.1 && 42.6 & 43.0 & 40.3 && 42.1 & 43.7 & 42.5 \\
% \textbf{flan-alpaca-gpt4-xl} && 76.6 & 79.6 & 37.2 && 80.5 & 78.3 & 22.6 && 60.4 & 91.8 & 65.9 \\
% \textbf{flan-t5-large} && 61.0 & 56.9 & 23.0 && 72.4 & 64.6 & 32.8 && 38.3 & 90.4 & 54.9 \\
% \textbf{flan-t5-xl} && 70.5 & 77.9 & 42.4 && 82.5 & 77.6 & 30.0 && 54.7 & 92.9 & 66.1 \\
% \textbf{flan-t5-base} && 13.2 & 15.6 & 6.3 && 15.3 & 12.6 & 5.9 && 13.6 & 10.3 & 11.6 \\
% \textbf{unifiedqa-v2-t5-large} && 61.7 & 59.8 & 28.8 && 71.3 & 63.7 & 27.4 && 50.3 & 75.2 & 54.8 \\
% \textbf{flan-t5-small} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{alpaca-lora-7b} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{falcon-7b-instruct} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-3.5-turbo} && - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-4} && - & - & - && - & - & - && - & - & - \\

% \midrule
%  && \multicolumn{9}{c}{\textbf{Combined (overall/positive/negative)}} \\
%  \midrule

%  \textbf{dolly-v2-7b} && 35.8 & 34.5 & 34.4 && 37.0 & 35.4 & 32.1 && 33.5 & 34.6 & 34.7 \\
% \textbf{flan-alpaca-gpt4-xl} && 64.9 & 70.4 & 43.7 && 69.9 & 67.4 & 36.5 && 54.2 & 79.1 & 60.8 \\
% \textbf{flan-t5-large} && 51.2 & 48.5 & 33.9 && 46.6 & 57.1 & 31.5 && 38.6 & 69.9 & 47.3 \\
% \textbf{flan-t5-xl} && 65.6 & 69.0 & 46.6 && 73.9 & 75.6 & 41.2 && 57.1 & 85.3 & 64.4 \\
% \textbf{flan-t5-base} && 36.2 & 34.3 & 27.7 && 32.3 & 33.9 & 28.7 && 33.2 & 33.9 & 34.1 \\
% \textbf{unifiedqa-v2-t5-large} && 53.6 & 55.7 & 39.6 && 64.3 & 62.3 & 39.5 && 50.0 & 64.1 & 53.7 \\
% \textbf{flan-t5-small} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{alpaca-lora-7b} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{falcon-7b-instruct} &&  - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-3.5-turbo} && - & - & - && - & - & - && - & - & - \\
% \textbf{GPT-4} && - & - & - && - & - & - && - & - & - \\

% % \textbf{Model W} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
% % \textbf{Model V} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
% \bottomrule
% \end{tabular}

% }

% \end{center}
% \caption{\textbf{Fundamental attribute understanding.}}
% \label{tab:fundamental_attribute_understanding}
% \end{table*}

% \begin{center}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l p{0.2pt}ccc p{0.2pt}ccc p{0.2pt}ccc}
%     \toprule
%     \textbf{Language Model} && Elasticity & Stiffness & Surface Smoothness && Surface Hardness & Softness & Brittleness && Malleability & Sharpness & Overall \\
%         \cline{3-13}

%       && \multicolumn{9}{c}{\textbf{Boolean (positive/negative)}} \\

%     \midrule

    
    
%     \textbf{xlnet-large-cased} && 38.3 & 32.7 & 31.5 && 31.1 & 39.1 & 28.6 && 35.5 & 27.6 & 33.8 \\
%     \textbf{xlm-roberta-large} && 37.1 & 23.1 & 33.6 && 21.5 & 36.7 & 40.6 && 32.2 & 23.1 & 32.3 \\
%     \textbf{roberta-large} && 27.0 & 24.4 & 37.7 && 22.6 & 37.4 & 48.6 && 34.5 & 34.8 & 34.5 \\
%     \textbf{bert-large-uncased} && 32.9 & \textbf{42.2} & 28.1 && 39.8 & 38.6 & 25.0 && 23.9 & 31.1 & 31.7 \\
%     \textbf{albert-xxlarge-v2} && 36.4 & 27.9 & \textbf{41.1} && 26.9 & 41.3 & 8.3 && 18.6 & 23.4 & 27.9 \\
    
%     \textbf{GPT-3.5-turbo} &&  26.4 & 0.0 & 1.4 && 16.1 & 7.8 & 7.6 && \textbf{68.8}  & 0.2 & 19.8 \\
%     \textbf{GPT-4} && \textbf{55.7} & 12.2 & 20.0 && \textbf{54.8} & \textbf{67.6} & \textbf{91.3} && 52.1 & \textbf{66.3} & \textbf{58.3} \\

%     \midrule
%      && \multicolumn{9}{c}{\textbf{Multiple Choice (positive/negative)}} \\
%      \midrule

%      \textbf{xlnet-large-cased} && 38.3 & 32.7 & 31.5 && 31.1 & 39.1 & 28.6 && 35.5 & 27.6 & 33.8 \\
%     \textbf{xlm-roberta-large} && 37.1 & 23.1 & 33.6 && 21.5 & 36.7 & 40.6 && 32.2 & 23.1 & 32.3 \\
%     \textbf{roberta-large} && 27.0 & 24.4 & 37.7 && 22.6 & 37.4 & 48.6 && 34.5 & 34.8 & 34.5 \\
%     \textbf{bert-large-uncased} && 32.9 & \textbf{42.2} & 28.1 && 39.8 & 38.6 & 25.0 && 23.9 & 31.1 & 31.7 \\
%     \textbf{albert-xxlarge-v2} && 36.4 & 27.9 & \textbf{41.1} && 26.9 & 41.3 & 8.3 && 18.6 & 23.4 & 27.9 \\
    
%     \textbf{GPT-3.5-turbo} &&  26.4 & 0.0 & 1.4 && 16.1 & 7.8 & 7.6 && \textbf{68.8}  & 0.2 & 19.8 \\
%     \textbf{GPT-4} && \textbf{55.7} & 12.2 & 20.0 && \textbf{54.8} & \textbf{67.6} & \textbf{91.3} && 52.1 & \textbf{66.3} & \textbf{58.3} \\
    
%     % \textbf{Model W} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     % \textbf{Model V} && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{center}
% \caption{\textbf{Fundamental attribute understanding.}.}
% \label{tab:fundamental_attribute_understanding}
% \end{table*}


% \subsection{How do language models compare with humans in understanding physics attributes?}
% \subsection{How well do language models understand physics attributes of everyday objects?}
% \subsection{Are language models aware of the necessary attributes for answering scenario-based questions?}

% \subsection{Explicit vs. Implicit Reasoning}

% Insert figure
% \begin{figure*}
% \centering
% \includegraphics[width=0.8\linewidth]{sections/images/ablation2.png}
% \caption{}
% \label{fig:accuracy-polarity}
% \end{figure*}

% \begin{figure*}
% \centering
% \includegraphics[width=\linewidth]{sections/images/ablation.png}
% \caption{}
% \label{fig:ablation}
% \end{figure*}


% Difficult to separate the results from the prompting method, perhaps different language models are suited to different ways of prompting, and hence using the same method of prompting may yield biased results.
% This suggests the promising ability for language models to reason about object attributes in an implicit manner, 


% and prompts thought on methods to improve its explicit understanding

% \subsection{\dataset Extensions}
% In this section, we provide an analysis of other potential ways of leveraging \dataset, particularly related to endowing language models with a better sense of physical reasoning through finetuning, and leveraging \dataset through the GPT-3.5-Turbo Function call.

% \noindent \textbf{Fine-tuning using \dataset.} It is hypothesized that with the rich set of object-attribute pairs which \dataset provides, we can endow language models with physical reasoning by finetuning in an explicit manner, such that performance for downstream implicit tasks is improved. To test this hypothesis, we fine-tune the base BERT model for the multiple choice task. The baseline consists of the base BERT model \cite{devlin2019bert}, fine-tuned on the SWAG dataset for multiple choice inference \cite{zellers2018swag}. The finetuning process uses subsets of \dataset QA - explicit reasoning track \{5000, 10000, 40000\}, and all models are evaluated on the implicit reasoning task, provided by the \dataset QA Implicit Reasoning Track. As shown in Figure \ref{fig:ablation} e find that including \dataset as a part of the pre-training procedure vastly improves performance on downstream implicit reasoning tasks, demonstrating the potential of leveraging \dataset for finetuning language models to improve their physical reasoning ability.

% \noindent \textbf{Using \dataset in Function Calls.}



% \begin{table*}[h]
% \centering
% \small
% \begin{tabularx}{\textwidth}{|l|l|X|X|X|}
% \hline
% \textbf{Property} & \textbf{Type} & \textbf{Definition} & \textbf{Question} & \textbf{Options} \\
% \hline
% Elasticity & Physics & Elasticity in this context refers to the ability of an object to recover to the original form after deformation. & If you were to deform \textless MASK\textgreater\ (by squeezing, hitting, etc.), can it recover to its original form? & No: Object will not be able to return to its original form. Somewhat: Object may recover to its original form but will have signs of previous deformations. Yes: Object is capable of recovering near perfectly to the original form. \\
% \hline
% Surface smoothness & Physics & Surface smoothness in this context refers to the texture of the outer surface of the object. & What is the surface smoothness of \textless MASK\textgreater? & Low: Majority of the surface is very rough or has many bumps. Moderate: Some parts of the surface are smooth, while some parts are not. High: Majority of the surface is smooth. \\
% \hline
% Surface Hardness & Physics & Surface hardness in this context refers to the ability of a surface to resist damage. & How resistant to scratches or bruises is the surface of \textless MASK\textgreater? & Low: The surface can be easily scratched or bruised. Moderate: The surface is resistant to most unintentional damage but could be scratched if force is applied. High: The object does not get scratched or bruised easily. \\
% \hline
% Brittleness & Physics & Brittleness in this context refers to the resistance of objects to sudden forces. & How easy is it for \textless MASK\textgreater\ to break (shatter, crack) when a sudden impact force is applied? & Low: The object can withstand most impact forces (drop, smash, etc.). Moderate: The object can withstand minor impact forces. High: The object shatters easily with impact force. \\
% \hline
% Softness & Physics & Softness refers to the fluffiness and squishiness of the external and internal composition of an object. & What is the softness (fluffiness, squishiness) of \textless MASK\textgreater? & Low: The object is hard. Moderate: Some parts of the object are soft. High: The majority of the object is soft. \\
% \hline
% Sharpness & Physics & Sharpness refers to the exterior design and material of an object. & What is the sharpness of \textless MASK\textgreater? & Low: The object does not have sharp corners/edges and is not capable of piercing. Moderate: The object may have sharp corners/edges but is not designed to pierce. High: The object is designed to pierce. \\
% \hline
% Stiffness & Physics & Stiffness refers to whether an object can withstand continued force without deforming or cracking. & What is the amount of continued weight that \textless MASK\textgreater\ can withstand before deforming or cracking? & Low: The object can support very minimal weight before deforming or cracking. Moderate: The object can withstand a small amount of weight, but something heavy (i.e., a 10 kg weight) will be able to deform or break the object. High: The object can easily withstand more than a 10 kg weight. \\
% \hline
% Malleability & Physics & Malleability refers to whether an object can be reshaped to take other geometries. & Can \textless MASK\textgreater\ be reshaped into other forms? & No: The object cannot be reshaped. Somewhat: The object can be slightly reshaped. Yes: The object can be reshaped into most arbitrary forms. \\
% \hline
% \end{tabularx}
% \caption{Properties of Objects}
% \label{tab:object_properties}
% \end{table*}

